Subspace Mixed-FEM for Real-Time Heterogeneous Elastodynamics

We propose a reduced space mixed finite element method (MFEM) built on a Skinning Eigenmode subspace and material-aware cubature scheme. Our solver is well-suited for simulating scenes with large material and geometric heterogeneities in real-time. This mammoth geometry is composed of 98,175 vertices and 531,565 tetrahedral elements and with a heterogenous composition of widely varying materials of muscles ($E= 5\times10^5$ Pa), joints ($E=1\times10^5$ Pa), and bone ($E=1\times10^{10}$ Pa). The resulting simulation runs at 120 frames per second (FPS).

==> background.tex <==


\section{Full Space Mixed-FEM}

Continuous Energy:
\begin{align}
    E(x) = \int_\Omega  \psi(x)  d\Omega
\end{align}
Energy can be rewritten more simply in terms of stretches :
\begin{align}
    E(x) = \int_\Omega  \psi(x, \bar{S}(x))  d\Omega
\end{align}

Where we obtain the stretch matrix from a polar decomposition of the deformation gradient $F(x) = \nabla x = \bar{R}(x) \bar{S}(x)$.

Minimize energy above for $\x$
\begin{align}
x^* =  \argmin_{x} \int_\Omega  \psi(x, \bar{S}(x))  d\Omega
\end{align}
Instead, add auxillary degrees of freedom for stretch variables and change the optimization to:
\begin{align}
x^*, S^* =  \argmin_{x, S} \int_\Omega  \psi(x, S)  d\Omega \quad \textrm{s.t.} \quad \bar{S}(x) = S 
\end{align}

Most energies can then be decomposed cleanly, with two independant energies written in terms $x$, and $S$ : 
\begin{align}
x^*, S^* =  \argmin_{x, S} \int_\Omega  \psi_x(x) + \psi_S(S)  d\Omega \quad \textrm{s.t.} \quad \bar{S}(x) = S
\end{align}

We can then enforce the constraint via Lagrange multipliers, introducing a diagonal matrix of lagrange multipliers $\Lambda$:
\begin{align}
x^*, S^*, \Lambda ^* =  \saddle_{x, S; \Lambda} \int_\Omega  \psi_x(x) + \psi_S(S) + \Lambda : (\bar{S}(x) - S) d\Omega
\end{align}

We then take advantage of the fact that 
$S$ and $\bar{S}$ are both symmetric, so we can rewrite both of these by cutting out  half of the non-diagonal terms, and placing the remainder in $\s$ and $\bar{s}$, and a diagonal matrix $D$ that weighs each term ( off diagonal terms are now representing two entries from the original constraint):

\begin{align}
x^*, s^*, \lambda ^*  =  \saddle_{x, s; l}  \int_\Omega  \psi_x(x) + \psi_s(s) + \lambda^T D (\bar{s} - s)  d\Omega
\end{align}

We can discretize our domain with linear finite elements, where positions $\x \in \Rn{(\dim)n  \times 1} $ are stored piece-wise linearly at nodes, and stretch degrees of freedom   $\s \in \Rn{ \frac{\dim(\dim +1 ) t}{2}  \times 1} $ are stored piece-wise constantly in elements. Our optimization becomes:

\begin{align}
\x^*, \s^*, \l^*  =  \saddle_{\x, \s; \l}   \Psi_x(x) + \Psi_s(\s) + \l^T \D (\bar{\s} - \s)  
\label{eq:mfem-discrete-optimization}
\end{align}

Solving for each of these variables using newton's method gives us the KKT system of equations to solve for a search direction:

\begin{align}
        \begin{bmatrix}
        \Hx & \0 & \Gx \\
        \0   & \Hs & \Gs \\
        \Gx^T & \Gs^T & \0
        \end{bmatrix}
        \begin{bmatrix}
        \dx \\ \ds \\ \dl
        \end{bmatrix}
        =
        \begin{bmatrix}
        \fx \\ \fs \\ \fl
        \end{bmatrix}
\end{align}

Where $ \Gx = \D \pderiv{\bar{s}}{\x} $, and $ \Gs = -\D \pderiv{s}{\s} = -\D $ are the derivative of our constraint with respect to $\x$ and $\s$ respectively. $\Hx= \pdderiv{\Psi_x}{\x}$, and $\Hs=\pdderiv{\Psi_s}{\s}$ are the Hessians, while $\fx = -\pderiv{\Psi_x}{\x} - \Hx \x $ and $\fs =  -\pderiv{\Psi_s}{\s} - \Hs \s$ are the gradients of  both energies $\Psi_x$ and $\Psi_s$ respectively at Newton iteration $i$.

We can do a couple Schur Complement tricks to obtain two systems that are much easier to solve for both $\dx$ and $\ds$.

\begin{align}
(\Hx + \L ) \dx &= \fx + \K \fl - \Gx^T \Gs^{-T} \fs \\
\ds &= \Gs^{-1}(\fl - \Gx \dx)
\end{align}

Where we used $\L = \Gx^T \Gs^{-T} \Hs \Gs^{-1} \Gx $ and $\K =  \Gx^T \Gs^{-T} \Hs \Gs^{-1} $






\section{Subspace Mixed FEM}
We introduce a linear subspace for our positional degrees of freedom: $\x  \approx \B \u$
With this in hand, we can replace our positional degrees of freedom with our subspace and rewrite \refeq{mfem-discrete-optimization}:

\begin{align}
\u^*, \s^*, \l^*  =  \saddle_{\u, \s; \l}   \Psi_u(u) + \Psi_s(\s) + \l^T \D (\bar{\s} - \s)  
\label{eq:mfem-discrete-optimization-reduced}
\end{align}
Note however, that our stretch variables $\s$, which need to be evaluated for both the second energy term and the constraint still live in the full space.  To decouple the simulation above fully from mesh complexity, we need a strategy to approximate the second energy term and the constraint. Thus, we introduce a cubature approximation for both these terms. 
\begin{align}
    \Psi_s(\s)  = \sum_t^{\numtets} \psi_s(\s_t) 
     \approx \sum_c^{\numcubature} w_c \psi(\z_c) = \Psi_z(\z) \\  
    \l^T \D (\bar{\s} - \s)   = \sum_t^{\numtets} \l_t^T \D_t (\bar{\s}_t - \s_t)  \approx &\sum_c^{\numcubature}  w_c \lxi_c ^T\D_c (\bar{\z}_c - \z_c) \nonumber  \\ =& \lxi^T \D  \Q (\bar{\z} - \z) 
\end{align}

Where we have introduced $\Q$, a diagonal matrix of cubature weights.


This finally lets us rewrite the optimization problem entirely in terms of reduced space degrees of freedom.
\begin{align}
\u^*, \z^*, \lxi^*  =  \saddle_{\u, \z; \lxi}   \Psi_u(u) + \Psi_z(\z) + \lxi^T \D  \Q (\bar{\z} - \z) 
\label{eq:mfem-discrete-optimization-reduced}
\end{align}

Each Newton iteration, the final hyper-reduced KKT system becomes:
\begin{align}
        \begin{bmatrix}
        \Hu & \0 & \Gu \\
        \0   & \Hz & \Gz \\
        \Gu^T & \Gz^T & \0
        \end{bmatrix}
        \begin{bmatrix}
        \du \\ \dz \\ \lxi
        \end{bmatrix}
        =
        \begin{bmatrix}
        \fu \\ \fz \\ \fxi
        \end{bmatrix}
\end{align}

Where $\Hu = \B^T\Hx \B$, and $\Hz = \Q \P^T\Hs \P$ are our reduced Hessians, $\fu = \B^T\fx$  and $\fz = \Q \P^T\fs$ are our reduced forces, $\Gu= \D \Q \pderiv{\bar{\z}}{\u} $ and  $\Gz= -\D \Q \pderiv{\z}{\z} = -\D \Q  $ are our reduced space constraint gradients.


We also make use of $\P $, a stretch subspace matrix that maps from our subspace stretches $\z$, to our full space stretches $\s$. In standard cubature, this amounts to just being a cubature selection matrix.

We can again carefully rewrite this system in terms of two smaller ones that are easier to solve:
\begin{align}
(\Hu + \L ) \du &= \fu + \K \fxi - \Gu^T \Gz^{-T} \fz \\
\dz &= \Gz^{-1}(\fxi - \Gu \dz)
\end{align}

Where we have again introduced temporary matrices for clarity: $\L = \Gu^T \Gz^{-T} \Hs \Gz^{-1} \Gu $ and $\K =  \Gu^T \Gz^{-T} \Hs \Gz^{-1} $



\section{Subspace Construction}
\subsection{Skinning Eigenmode Subspace}
There are many ways to construct $\B$. We opt for using Skinning Eigenmodes as they have been shown to provide modes that represent rotational properties essential for stiff materials, while also providing material sensitivity.

Specifically, we obtain a set of skinning weights by solving the weight space generalized eigenvalue problem:
\begin{align}
    \Hw \W = \Mw \W \boldsymbol{\Gamma}
\end{align}
Where $\Hw$ is the weight space Hessian (The sum of the 3 diagonal blocks of elastic energy Hessian), and $\Mw$ is the scalar Mass matrix.
These skinning weights $\W$ can then be used to construct our subspace basis $\B$ using the standard linear blend skinning Jacobian:
\begin{align}
    \B = \I_{\dim}  \otimes (  ( \boldsymbol{1}_b^T \otimes \bar{\X} ) \odot  ( \W \otimes  \boldsymbol{1}_{\dim + 1}^T ))
\end{align}
Where $\bar{\X} \in \Rn{n \times \dim +1}$ are our rest positions in homogeneous coordinates.  

\subsection{Cubature Construction}

To sample cubature tetrahedra, we cluster our domain and choose the tetrahedra closest to the centroid of each cluster. 

We construct these clusters from a kmeans clustering on our skinning weights. This groups tetrahedra togather share the similar skinning weights. 

\begin{align}
    l = \mathrm{kmeans}(\W_{\mathcal{T}}\Lambda^{-2}, \mathrm{k})
\end{align}

Where $\W_{\mathcal{T}}$ are our skinning weights averaged from the vertices to the tets. We weigh each skinning weight by its inverse squared eigenvalue to more heavily favor lower order skinning eigenmodes in our clustering scheme. We can then easily compute cluster centroids and choose our cubature points as the tets closest to each centroid.

The cubature weights can then trivially be computed as the mass of each cluster.



==> limitations.tex <==
\section{Limitations and Future Work}


==> regularization.tex <==

\section{ Ty's Cubature Consistency Regularization }
Because cubature/clustering can severley underintegrate our energy, they can introduce spurious low energy motions, that incur now measured subspace elastic energy, but have a very jarring visual impact on the simulation.

To help fix this, we propose to add a regularization penalty term:

\begin{align}
    E_{\mathrm{reg}}(x) =  \sum_c^{\numcubature} \gamma_c   \sum_c^{\numtets}   w_{tc}|| F_t -    F_c||^2_F
\end{align}

Where $w_{tc}$ is a membership variable (randing from 0 to 1) that indicates how much a tet belongs to each cluster, and $\gamma_t$ is a user defined value greater than zero that weighs our regularization term.

This regularization term pushes each tet's deformation gradient to be as close as possible to a weighed average of the cubature points deformation gradients.

So far, we have only considered a simplified version of this penalty term, where each tet is mapped to its closest cubature point and only attempts to match that deformation gradient in isolation.

\section{Otman's Quadratic Refactoring }
The idea is that when we are approximating the cubature the non-linear energy term, we are needlessly approximating a large part of this integral. 

For example, consider the ARAP energy density, which we can rewrite  in terms of our stretches:

\begin{align}
     \Psi_{ARAP}(\S) =  \sum_t^{\numtets} m_t \mu_t || \S_t - \I ||_{F}^2 
\end{align}

We currently approximate this entire energy using cubature:
\begin{align}
     \approx  \sum_t^{\numcubature} w_c \mu_c || \Z_c - \I ||_{F}^2 
\end{align}

Is it really necessary to do such a heavy handed approximation? Let's massage the full space ARAP energy and see if there are any terms we can fully integrate within our subspace.
\begin{align}
     \Psi_{ARAP}(\S)  =  \sum_t^{\numtets} m_t \mu_t || \S_t - \I ||_{F}^2 = \sum_t^{\numtets} m_t \mu_t (tr(\S_t^T\S_t) - 2 tr(\S_t) + tr(\I))
\end{align}

Plugging in our constraint $\S_t = \bar{\S}_t(\x) = \R^T_t F_t$ and updating the first term:

\begin{align}
     \Psi_{ARAP} &=  \sum_t^{\numtets} m_t \mu_t || \S_t - \I ||_{F}^2 = \sum_t^{\numtets} m_t \mu_t (tr(F_t^T \underbrace{\R_t\R^T_t}_{\I} \F_t) - 2 tr(\S_t) + tr(\I)) \nonumber \\
    &= \sum_t^{\numtets} m_t \mu_t ( \underbrace{tr(\F_t^T  \F_t)} - 2 tr(\S_t) + tr(\I)) 
\end{align}
Note that the underbrace component is \emph{quadratic} in our positional degrees of freedom, which means it is quadratic in our positional subspace degrees of freedom as well. It can be rewritten in terms of our subspace dofs:

\begin{align}
    \sum_t^{\numtets} m_t \mu_t tr(\F_t^T  \F_t) =   \u  \underbrace{\B^T \J^T \A \mathcal{U} \J }\B  \u
\end{align}
With $\A$ being a diagonal tet volume matrix, $\mathcal{U}$ is a diagonal second Lame parameter matrix, $\J$ is the deformation Jacobian matrix, and $\B$ is the subspace matrix.  Note that the underbraced matrix is \emph{constant} and so the resulting contribution to the energy can be evaluated at run-time in sub-full space complexity.

So the proposal is to move this component of the energy $\Psi_u$, essentially reduced the amount of our our cubatured $\Psi_z$ has to do in our approximation.

We then have a modified $\tilde{\Psi}_u$ and $\tilde{\Psi}_z$:


\begin{align}
    \tilde{\Psi}_x &= \Psi_x +  \x^T  \J^T \A \mathcal{U} \J  \x \\
    \tilde{\Psi}_s &= - 2 \sum_t^{\numtets} \mu_t tr(\S_t)  
\end{align}



\begin{align}
    \tilde{\Psi}_u &= \Psi_u +  \u^T \B^T \J^T \A \mathcal{U} \J \B  \u \\
    \tilde{\Psi}_z &= - 2 \sum_c^{\numcubature} w_c \mu_c tr(\Z_c)  
\end{align}



